SpINR: Neural Volumetric Reconstruction for FMCW Radars

In this paper, we introduce SpINR, a novel framework for volumetric reconstruction using Frequency-Modulated Continuous-Wave (FMCW) radar data. Traditional radar imaging techniques, such as backprojection, often assume ideal signal models and require dense aperture sampling, leading to limitations in resolution and generalization. To address these challenges, SpINR integrates a fully differentiable forward model that operates natively in the frequency domain with implicit neural representations (INRs). This integration leverages the linear relationship between beat frequency and scatterer distance inherent in FMCW radar systems, facilitating more efficient and accurate learning of scene geometry. Additionally, by computing outputs for only the relevant frequency bins, our forward model achieves greater computational efficiency compared to time-domain approaches that process the entire signal before transformation. Through extensive experiments, we demonstrate that SpINR significantly outperforms classical backprojection methods and existing learning-based approaches, achieving higher resolution and more accurate reconstructions of complex scenes. This work represents the first application of neural volumetic reconstruction in the radar domain, offering a promising direction for future research in radar-based imaging and perception systems.

==> background.tex <==
\section{Background and Motivation (Volumetric reconstruction with mmWave Radar)}

The goal is to perform 3D scene reconstruction from commercially available mmWave sensors that are generally used as automotive radars. We assume non-uniformly sampled mmWave sensor recordings.

\subsection{Traditional 3D reconstruciton}
Camera- prone to ambient light conditions

\subsection{Image formation model}

The chirp can be represented as 

\[
m(t) = \cos\left(2\pi\left(f_0 t + 0.5 K t^2\right)\right), \quad 0 \leq t \leq T,
\]

where $f_0$ is the carrier frequency at time $t = 0$, $K = \frac{B}{T}$ is the slope of frequency computed from the sweep bandwidth $B$, and $T$ is the chirp duration.
The reflected chirp can be represented as

\[
\hat m(t) = \sigma m(t-\tau)  = \sigma\cos\left(2\pi\left(f_0 (t-\tau) + 0.5 K (t-\tau)^2\right)\right), \quad 0 \leq t \leq T,
\]
where $\tau$ is the round-trip delay of the echo and $\sigma$ is the combination of target reflectivity and the round-trip amplitude decay off the target.

The distance estimate can then be found by taking the range FFT of the received signal

\[
FFT(\hat m(t))
\]

Each fft bin corresponds to range by the relation - 

This only gives us a resolution of 4.16 cm. To increase the resolution beyond this, we need to leverage the phase component.

\subsection{FMCW Radars}
In a Frequency Modulated Continuous Wave (FMCW) radar, transmits a wave whose frequency varies linearly over time. The transmitted signal reflects off targets, and the radar receives these echoes with a time delay corresponding to the target's distance. By mixing the received signal with a portion of the transmitted signal, the system generates a beat frequency proportional to the range of the target. This beat frequency is analyzed to determine the target's distance and relative velocity.



\begin{equation}
p(x,y,z) = \iiiint s(x,y_T, y_R, k)  e^{jkR_T} e^{jkR_R} dx dy_T dy_R  dk
\end{equation}


\subsection{Implicit Neural Represenataion}



==> body.tex <==

% Head 1
\section{MMSN Protocol}

% Head 2
\subsection{Frequency Assignment}

We propose a suboptimal distribution to be used by each node, which is
easy to compute and does not depend on the number of competing
nodes. A natural candidate is an increasing geometric sequence, in
which
% Numbered Equation
\begin{equation}
\label{eqn:01}
P(t)=\frac{b^{\frac{t+1}{T+1}}-b^{\frac{t}{T+1}}}{b-1},
\end{equation}
where $t=0,{\ldots}\,,T$, and $b$ is a number greater than $1$.

In our algorithm, we use the suboptimal approach for simplicity and
generality. We need to make the distribution of the selected back-off
time slice at each node conform to what is shown in
Equation~\eqref{eqn:01}. It is implemented as follows: First, a random
variable $\alpha$ with a uniform distribution within the interval $(0,
1)$ is generated on each node, then time slice $i$ is selected
according to the following equation:
% Unnumbered Equation
\[
i=\lfloor(T+1)\log_b[\alpha(b-1)+1]\rfloor.
\]
It can be easily proven that the distribution of $i$ conforms to Equation
(\ref{eqn:01}).

So protocols \cite{Tzamaloukas-01, Akyildiz-01, Adya-01, Bahl-02, Culler-01,Zhou-06} that use RTS/CTS
controls\footnote{RTS/CTS controls are required to be implemented by
802.11-compliant devices. They can be used as an optional mechanism
to avoid Hidden Terminal Problems in the 802.11 standard and
protocols based on those similar to \cite{Akyildiz-01} and
\cite{Adya-01}.} for frequency negotiation and reservation are not
suitable for WSN applications, even though they exhibit good
performance in general wireless ad-hoc
networks.

% Head 3
\subsubsection{Exclusive Frequency Assignment}


In exclusive frequency assignment, nodes first exchange their IDs
among two communication hops so that each node knows its two-hop
neighbors' IDs. In the second broadcast, each node beacons all
neighbors' IDs it has collected during the first broadcast period.

% Head 4
\paragraph{Eavesdropping}

Even though the even selection scheme leads to even sharing of
available frequencies among any two-hop neighborhood, it involves a
number of two-hop broadcasts. To reduce the communication cost, we
propose a lightweight eavesdropping scheme.

\subsection{Basic Notations}

As Algorithm~\ref{alg:one} states, for each frequency
number, each node calculates a random number (${\textit{Rnd}}_{\alpha}$) for
itself and a random number (${\textit{Rnd}}_{\beta}$) for each of its two-hop
neighbors with the same pseudorandom number generator.

% Algorithm
\begin{algorithm}[t]
\SetAlgoNoLine
\KwIn{Node $\alpha$'s ID ($ID_{\alpha}$), and node $\alpha$'s
neighbors' IDs within two communication hops.}
\KwOut{The frequency number ($FreNum_{\alpha}$) node $\alpha$ gets assigned.}
$index$ = 0; $FreNum_{\alpha}$ = -1\;
\Repeat{$FreNum_{\alpha} > -1$}{
        $Rnd_{\alpha}$ = Random($ID_{\alpha}$, $index$)\;
        $Found$ = $TRUE$\;
        \For{each node $\beta$ in $\alpha$'s two communication hops
    }{
      $Rnd_{\beta}$ = Random($ID_{\beta}$, $index$)\;
      \If{($Rnd_{\alpha} < Rnd_{\beta}$) \text{or} ($Rnd_{\alpha}$ ==
          $Rnd_{\beta}$ \text{and} $ID_{\alpha} < ID_{\beta}$)\;
      }{
        $Found$ = $FALSE$; break\;
      }
        }
     \eIf{$Found$}{
           $FreNum_{\alpha}$ = $index$\;
         }{
           $index$ ++\;
     }
      }
\caption{Frequency Number Computation}
\label{alg:one}
\end{algorithm}


Bus masters are divided into two disjoint sets, $\mathcal{M}_{RT}$
and $\mathcal{M}_{NRT}$.
% description
\begin{description}
\item[RT Masters]
$\mathcal{M}_{RT}=\{ \vec{m}_{1},\dots,\vec{m}_{n}\}$ denotes the
$n$ RT masters issuing real-time constrained requests. To model the
current request issued by an $\vec{m}_{i}$ in $\mathcal{M}_{RT}$,
three parameters---the recurrence time $(r_i)$, the service cycle
$(c_i)$, and the relative deadline $(d_i)$---are used, with their
relationships.
\item[NRT Masters]
$\mathcal{M}_{NRT}=\{ \vec{m}_{n+1},\dots,\vec{m}_{n+m}\}$ is a set
of $m$ masters issuing nonreal-time constrained requests. In our
model, each $\vec{m}_{j}$ in $\mathcal{M}_{NRT}$ needs only one
parameter, the service cycle, to model the current request it
issues.
\end{description}

Here, a question may arise, since each node has a global ID. Why
don't we just map nodes' IDs within two hops into a group of
frequency numbers and assign those numbers to all nodes within two
hops?

\section{Simulator}
\label{sec:sim}

If the model checker requests successors of a state which are not
created yet, the state space uses the simulator to create the
successors on-the-fly. To create successor states the simulator
conducts the following steps.
% enumerate
\begin{enumerate}
\item Load state into microcontroller model.
\item Determine assignments needed for resolving nondeterminism.
\item For each assignment.
      \begin{enumerate}
      \item either call interrupt handler or simulate effect of next instruction, or
      \item evaluate truth values of atomic propositions.
      \end{enumerate}
\item Return resulting states.
\end{enumerate}
Figure~\ref{fig:one} shows a typical microcontroller C program that
controls an automotive power window lift. The program is one of the
programs used in the case study described in Section~\ref{sec:sim}.
At first sight, the programs looks like an ANSI~C program. It
contains function calls, assignments, if clauses, and while loops.
% Figure
\begin{figure}
  \includegraphics{Figures/mouse}
  \caption{Code before preprocessing.}
  \label{fig:one}
\end{figure}

\subsection{Problem Formulation}

The objective of variable coalescence-based offset assignment is to find
both the coalescence scheme and the MWPC on the coalesced graph. We start
with a few definitions and lemmas for variable coalescence.

% Enunciations
\begin{definition}[Coalesced Node (C-Node)]A C-node is a set of
live ranges (webs) in the AG or IG that are coalesced. Nodes within the same
C-node cannot interfere with each other on the IG. Before any coalescing is
done, each live range is a C-node by itself.
\end{definition}

\begin{definition}[C-AG (Coalesced Access Graph)]The C-AG is the access
graph after node coalescence, which is composed of all C-nodes and C-edges.
\end{definition}

\begin{lemma}
The C-MWPC problem is NP-complete.
\end{lemma}
\begin{proof} C-MWPC can be easily reduced to the MWPC problem assuming a
coalescence graph without any edge or a fully connected interference graph.
Therefore, each C-node is an uncoalesced live range after value separation
and C-PC is equivalent to PC. A fully connected interference graph is made
possible when all live ranges interfere with each other. Thus, the C-MWPC
problem is NP-complete.
\end{proof}

\begin{lemma}[Lemma Subhead]The solution to the C-MWPC problem is no
worse than the solution to the MWPC.
\end{lemma}
\begin{proof}
Simply, any solution to the MWPC is also a solution to the
C-MWPC. But some solutions to C-MWPC may not apply to the MWPC (if any
coalescing were made).
\end{proof}

\section{Performance Evaluation}

During all the experiments, the Geographic Forwarding (GF) by Akyildiz
et al.~\shortcite{Akyildiz-01} routing protocol is used. GF exploits
geographic information of nodes and conducts local data-forwarding to
achieve end-to-end routing. Our simulation is configured according to
the settings in Table~\ref{tab:one}. Each run lasts for 2 minutes and
repeated 100 times. For each data value we present in the results, we
also give its 90\% confidence interval.

% Table
\begin{table}%
\caption{Simulation Configuration}
\label{tab:one}
\begin{minipage}{\columnwidth}
\begin{center}
\begin{tabular}{ll}
  \toprule
  TERRAIN\footnote{This is a table footnote. This is a
    table footnote. This is a table footnote.}   & (200m$\times$200m) Square\\ \midrule
  Node Number     & 289\\
  Node Placement  & Uniform\\
  Application     & Many-to-Many/Gossip CBR Streams\\
  Payload Size    & 32 bytes\\
  Routing Layer   & GF\\
  MAC Layer       & CSMA/MMSN\\
  Radio Layer     & RADIO-ACCNOISE\\
  Radio Bandwidth & 250Kbps\\
  Radio Range     & 20m--45m\\
  \bottomrule
\end{tabular}
\end{center}
\bigskip\centering
\footnotesize\emph{Source:} This is a table
 sourcenote. This is a table sourcenote. This is a table
 sourcenote.

 \emph{Note:} This is a table footnote.
\end{minipage}
\end{table}%


\section{Conclusions}

In this article, we develop the first multifrequency MAC protocol for
WSN applications in which each device adopts a
single radio transceiver. The different MAC design requirements for
WSNs and general wireless ad-hoc networks are
compared, and a complete WSN multifrequency MAC design (MMSN) is
put forth. During the MMSN design, we analyze and evaluate different
choices for frequency assignments and also discuss the nonuniform
back-off algorithms for the slotted media access design.

% Start of "Sample References" section

\section{Typical References in New ACM Reference Format}
A paginated journal article \cite{Abril07}, an enumerated
journal article \cite{Cohen07}, a reference to an entire issue \cite{JCohen96},
a monograph (whole book) \cite{Kosiur01}, a monograph/whole book in a series (see 2a in spec. document)
\cite{Harel79}, a divisible-book such as an anthology or compilation \cite{Editor00}
followed by the same example, however we only output the series if the volume number is given
\cite{Editor00a} (so Editor00a's series should NOT be present since it has no vol. no.),
a chapter in a divisible book \cite{Spector90}, a chapter in a divisible book
in a series \cite{Douglass98}, a multi-volume work as book \cite{Knuth97},
an article in a proceedings (of a conference, symposium, workshop for example)
(paginated proceedings article) \cite{Andler79}, a proceedings article
with all possible elements \cite{Smith10}, an example of an enumerated
proceedings article \cite{VanGundy07},
an informally published work \cite{Harel78}, a doctoral dissertation \cite{Clarkson85},
a master's thesis: \cite{anisi03}, an online document / world wide web
resource \cite{Thornburg01, Ablamowicz07, Poker06}, a video game (Case 1) \cite{Obama08} and (Case 2) \cite{Novak03}
and \cite{Lee05} and (Case 3) a patent \cite{JoeScientist001},
work accepted for publication \cite{rous08}, 'YYYYb'-test for prolific author
\cite{SaeediMEJ10} and \cite{SaeediJETC10}. Other cites might contain
'duplicate' DOI and URLs (some SIAM articles) \cite{Kirschmer:2010:AEI:1958016.1958018}.
Boris / Barbara Beeton: multi-volume works as books
\cite{MR781536} and \cite{MR781537}.

A couple of citations with DOIs: \cite{2004:ITE:1009386.1010128,
  Kirschmer:2010:AEI:1958016.1958018}.

Online citations: \cite{TUGInstmem, Thornburg01, CTANacmart}.



% DO NOT INCLUDE ACKNOWLEDGMENTS IN AN ANONYMOUS SUBMISSION TO SIGGRAPH 2019
%\begin{acks}
%
%The authors would like to thank Dr. Maura Turolla of Telecom
%Italia for providing specifications about the application scenario.
%
%The work is supported by the \grantsponsor{GS501100001809}{National
%  Natural Science Foundation of
%  China}{http://dx.doi.org/10.13039/501100001809} under Grant
%No.:~\grantnum{GS501100001809}{61273304\_a}
%and~\grantnum[http://www.nnsf.cn/youngscientists]{GS501100001809}{Young
%  Scientists' Support Program}.
%
%
%\end{acks}

% Bibliography
\bibliographystyle{ACM-Reference-Format}
\bibliography{sample-bibliography}

% Appendix
\appendix
\section{Switching Times}

In this appendix, we measure the channel switching time of Micaz
\cite{CROSSBOW} sensor devices.  In our experiments, one mote
alternatingly switches between Channels~11 and~12. Every time after
the node switches to a channel, it sends out a packet immediately and
then changes to a new channel as soon as the transmission is finished.
We measure the number of packets the test mote can send in 10 seconds,
denoted as $N_{1}$. In contrast, we also measure the same value of the
test mote without switching channels, denoted as $N_{2}$. We calculate
the channel-switching time $s$ as
\begin{displaymath}%
s=\frac{10}{N_{1}}-\frac{10}{N_{2}}.
\end{displaymath}%
By repeating the experiments 100 times, we get the average
channel-switching time of Micaz motes: 24.3\,$\mu$s.


==> conclusion.tex <==
\section{Conclusion}

==> evaluation.tex <==
\section{Evaluation}

\begin{figure*}[htbp]
  \centering
  \begin{tabular}{cccc}
    \includegraphics[width=0.22\textwidth]{Figures/ring/backprojected_scene_timedomain_render.png} & 
    \includegraphics[width=0.22\textwidth]{Figures/ring/backprojected_scene_freqdomain_render.png} &
    \includegraphics[width=0.22\textwidth]{Figures/ring/reconstructed_scene_Nerf_amp_render.png} &
    \includegraphics[width=0.22\textwidth]{Figures/ring/reconstructed_scene_Nerf_amp_phase_render.png} \\[6pt]
    
    \includegraphics[width=0.22\textwidth]{Figures/pyramid/bp_td_system_data_run42_6_render.png} & 
    \includegraphics[width=0.22\textwidth]{Figures/pyramid/bp_fd_system_data_run42_6_render.png} &
    \includegraphics[width=0.22\textwidth]{Figures/pyramid/final_upsampled_scene_reconstructed_scenes_242_4_render.png} &
    \includegraphics[width=0.22\textwidth]{Figures/pyramid/final_upsampled_scene_reconstructed_scenes_240_4_render.png} \\[6pt]

    \includegraphics[width=0.22\textwidth]{Figures/coffeemaker/bp_td_system_data_run32_5_render.png} & 
    \includegraphics[width=0.22\textwidth]{Figures/coffeemaker/bp_fd_system_data_run32_5_render.png} &
    \includegraphics[width=0.22\textwidth]{Figures/coffeemaker/final_upsampled_scene_reconstructed_scenes_241_2_render.png} &
    \includegraphics[width=0.22\textwidth]{Figures/coffeemaker/final_upsampled_scene_reconstructed_scenes_240_2_render.png} \\[6pt]

    \includegraphics[width=0.22\textwidth]{Figures/dog/bp_td_system_data_run37_5_render.png} & 
    \includegraphics[width=0.22\textwidth]{Figures/dog/bp_fd_system_data_run37_5_render.png} &
    \includegraphics[width=0.22\textwidth]{Figures/dog/final_upsampled_scene_reconstructed_scenes_241_1_render.png} &
    \includegraphics[width=0.22\textwidth]{Figures/dog/final_upsampled_scene_reconstructed_scenes_240_1_render.png} \\[6pt]

    \includegraphics[width=0.22\textwidth]{Figures/compound/bp_td_system_data_run28_5_render.png} & 
    \includegraphics[width=0.22\textwidth]{Figures/compound/bp_fd_system_data_run28_5_render.png} &
    \includegraphics[width=0.22\textwidth]{Figures/compound/final_upsampled_scene_reconstructed_scenes_241_3_render.png} &
    \includegraphics[width=0.22\textwidth]{Figures/compound/final_upsampled_scene_reconstructed_scenes_240_3_render.png} \\
  \end{tabular}
  \caption{A five-row by four-column grid of images. Replace filenames as needed.}
  \label{fig:5x4_images}
\end{figure*}


\subsection{Simualted Experiments}

\begin{figure}[H]
    % \centering
    \includegraphics[width=0.5\linewidth]{Figures/backprojected_data_2_point.png}
    \caption{Backprojected Data}
    \label{fig:enter-label1}
    \Description{A woman and a girl in white dresses sit in an open car.}
\end{figure}

\begin{figure}[H]
    % \centering
    \includegraphics[width=0.5\linewidth]{Figures/backprojected_data_4_point.png}
    \caption{Backprojected Data}
    \label{fig:enter-label2}
    \Description{A woman and a girl in white dresses sit in an open car.}
\end{figure}

\begin{figure}[H]
    % \centering
    \includegraphics[width=0.5\linewidth]{Figures/Nerf_output_two_point.png}
    \caption{Trained nerf output with lesser samples}
    \label{fig:enter-label3}
    \Description{A woman and a girl in white dresses sit in an open car.}
\end{figure}



\begin{figure}[H]
    % \centering
    \includegraphics[width=0.5\linewidth]{Figures/Nerf_output_four_point.png}
    \caption{Trained nerf output with lesser samples}
    \label{fig:enter-label4}
    \Description{A woman and a girl in white dresses sit in an open car.}
\end{figure}

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{Figures/mouse.pdf}
%   \caption{Architecture of our multimodal volume rendering model}
%   \label{architecture}
%   % \Description{A woman and a girl in white dresses sit in an open car.}
% \end{figure}

\subsection{Real World Experiments}

\subsubsection{Experiment setup} 
To build our real-world multimodal volumetric imaging system, we use millimeter wave (MMwave). Our setup leveraged the Texas Instruments AWR1843BOOST millimeter wave evaluation board with the DCA1000 data capture adapter as shown in Fig. \ref{mmsensor}. This FMCW-based sensor operates at 77GHz, providing high-resolution MMwave imaging capabilities. Our system consisted of a vertical actuator, on which the MMwave sensor was mounted, and a turntable, which held the object to be imaged as shown in the Fig.\ref{fullsetup}. The sensors were housed in a custom 3D-printed casing designed to ensure proper alignment and protection. The vertical actuator enabled precise vertical movement of the sensors, while the turntable facilitated rotational motion of the object, creating a synthetic aperture for comprehensive imaging.

==> experiment_setup.tex <==
\section{Experiment Setup}

To build our real-world volumetric imaging system, our setup leveraged the Texas Instruments AWR1843BOOST millimeter wave evaluation board with the DCA1000 data capture adapter as shown in Fig. \ref{mmsensor}. This FMCW-based sensor operates at 77GHz, providing high-resolution MMwave imaging capabilities. 

Our system consisted of a vertical actuator, on which the MMwave was mounted, and a turntable, which held the object to be imaged as shown in the Fig.\ref{fullsetup}. The sensors were housed in a custom 3D-printed casing designed to ensure proper alignment and protection. The vertical actuator enabled precise vertical movement of the sensors, while the turntable facilitated rotational motion of the object, creating a synthetic aperture for comprehensive imaging.

Accurate 3D positioning of the sensors is crucial for the effectiveness of the imaging system. Initial trials revealed inaccuracies in the actuator and turntable movements, which could compromise the imaging results. To address this issue, we employed a Vicon motion capture system for calibration. The Vicon system uses multiple cameras to track the precise location of passive infrared markers attached to the setup. This allowed us to calibrate the exact positions of the sensors, ensuring accurate data acquisition and enhancing the overall imaging accuracy.The combination of MMwave and acoustic sensors, along with precise actuator and turntable movements, enabled us to capture detailed volumetric images. 

==> introduction.tex <==
\section{Introduction}

Reconstruction of 3D shapes is a central challenge in vision - NERF has emerged as a solution.

Range scanning conventionally was performed with radars - recently mmwave radars have ben developed for automobiles that can perform range scanning. These use FMCW signals for their scanning. - these mmwave radar are used for vehicle detection, etc. -  they can also be used for imaging.

Sar imaging exist but has strict sampling constraints.


In this work we address the problem of reconstruction of 3D shapes with FMCW mmWave radar - we loosen the SAR minimum sampling distance constraint while maintaining high quality of reconstruction. We maintain the high reconstruction quality by modelling the FMCW signal in frequency domain. We model both the amplitude and phase of the freqeuncy domain signal



==> main_old.tex <==
\input{introduction}
\input{related_work}
\input{background}
\input{problem_statement}
\input{methods}
\input{experiment_setup}
\input{evaluation}
\input{conclusion}

==> methods.tex <==
\section{Method}
For a point scatterer at a distance d, the mixed beat signal can be defined as

\[
m(t) = \cos\left(2\pi\left(f_0 t + 0.5 K t^2\right)\right), \quad 0 \leq t \leq T,
\]





In our reconstruction framework, we represent the object's surface using a Signed Distance Function (SDF), $I(x,y,z)$, which outputs a distance of each 3D point  $(x,y,z)$ to the nearest surface




The intermediate frequency signal contains information about the distance of the scatterer from the sensor.


\section{Direct DFT calculation forward model} 
We model the FMCW  signal formation process directly in the frequency domain. For a known tramit signal, we model its interaction with the scene geometry. 



1. **Definition of a pure complex tone sequence:**

   \[
   S_n = M e^{i\left( f \cdot \frac{2\pi}{N} n + \phi \right)}
   \]

2. **Frequency rescaled to an angular measure:**

   \[
   \alpha = f \cdot \frac{2\pi}{N}
   \]

3. **Simplified form of the signal:**

   \[
   S_n = M e^{i(\alpha n + \phi)}
   \]

4. **Definition of the Discrete Fourier Transform (DFT):**

   \[
   Z_k = \frac{1}{N} \sum_{n=0}^{N-1} S_n e^{-i 2\pi \frac{k}{N} n}
   \]

5. **Angular frequency index substitution:**

   \[
   \beta_k = k \cdot \frac{2\pi}{N}
   \]

6. **DFT calculation with angular frequency substitution:**

   \[
   Z_k = \frac{1}{N} \sum_{n=0}^{N-1} S_n e^{-i \beta_k n}
   \]

7. **Definition of the Roots of Unity:**

   \[
   R_k = e^{-i \beta_k}
   \]

8. **Demonstration that \( R_k \) is an Nth Root of Unity:**

   \[
   R_k^N = \left( e^{-i \beta_k} \right)^N = \left( e^{-i \left( k \cdot \frac{2\pi}{N} \right)} \right)^N = \left( e^{-i 2\pi} \right)^k = 1^k = 1
   \]

9. **Substitution of the pure complex tone into the DFT definition:**

   \[
   Z_k = \frac{1}{N} \sum_{n=0}^{N-1} M e^{i(\alpha n + \phi)} e^{-i \beta_k n}
   \]

10. **Factoring out constants:**

    \[
    Z_k = \frac{M}{N} e^{i\phi} \sum_{n=0}^{N-1} e^{i(\alpha - \beta_k) n}
    \]

11. **Geometric summation formula:**

    \[
    \sum_{n=0}^{N-1} x^n = \frac{1 - x^N}{1 - x}
    \]

12. **Applying the summation formula to the DFT:**

    \[
    Z_k = \frac{M}{N} e^{i\phi} \cdot \frac{1 - e^{i(\alpha - \beta_k) N}}{1 - e^{i(\alpha - \beta_k)}}
    \]

13. **Noting that \( \beta_k N \) is a multiple of \( 2\pi \):**

    \[
    \beta_k N = k \cdot 2\pi
    \]

14. **Simplifying the numerator:**

    \[
    Z_k = \frac{M}{N} e^{i\phi} \cdot \frac{1 - e^{i\alpha N}}{1 - e^{i(\alpha - \beta_k)}}
    \]

15. **Condition when \( f \) is an integer frequency:**

    \[
    \alpha N = f \cdot 2\pi
    \]





\section{Frequency bin interpolation}
The range resolution frequency evaluation is limited by the available bandwidth. However, if we wish to incorporate the phase information to estimate the range, the output of the frequency evaluation needs to be better than $\lambda/2$

The complex representation of the beat signal:
\begin{equation}
y_k = \frac{1}{2} e^{j\phi_B} e^{j 2 \pi f_B k \Delta t}, \quad k = 0, \dots, N-1.
\end{equation}

The Discrete Fourier Transform (DFT) of the beat signal:
\begin{equation}
Y_n = \sum_{k=0}^{N-1} y_k e^{-j \frac{2 \pi kn}{N}}, \quad n = 0, \dots, N-1.
\end{equation}

The real beat frequency can be expressed as:
\begin{equation}
f_B = m \Delta f + q \Delta f, \quad \text{with } |Y_m| = \max_n |Y_n|, \quad q \in \left[-\frac{1}{2}, +\frac{1}{2}\right].
\end{equation}

The ratio for neighboring amplitudes:
\begin{equation}
A_{\pm 1} = \frac{Y_m - Y_{m \pm 1}}{Y_m} = 1 - \frac{Y_{m \pm 1}}{Y_m}.
\end{equation}

The absolute value of this ratio:
\begin{equation}
|A_{\pm 1}| = \frac{\sin \frac{\pi}{N}}{\left|\sin \left[\frac{\pi}{N}(1 - q)\right]\right|},
\end{equation}
which simplifies to:
\begin{equation}
|A_{\pm 1}| = \frac{1}{1 \pm q}.
\end{equation}

The residual part \( q \) is determined as:
\begin{equation}
q = \frac{|A_{+1}| - 1}{|A_{+1}|}, \quad q = \frac{1 - |A_{-1}|}{|A_{-1}|}.
\end{equation}


\section{Phase information}
Once we are within the unambigious range $R_{unamb}$ of $\lambda/2$, we can leverage the phase information to gain additional accuracy

\begin{equation}
    \Delta \phi_{IF}(\tau) = 2\pi f_{min} \tau
\end{equation}
\begin{equation}
    \Delta R = R_{umabl} \frac{\phi}{180} 
\end{equation}

\subsection{Forward Model}

\subsubsection{two step forward model}

\subsection{Unwrapping phase}

\subsection{Colocated Tx-Rx/ spherical sampling}

\subsection{chirps/ frames/ collection parameters}

\subsection{calibration}

\subsection{ISAR}



\subsection{Non Uniform Sampling}
Once we obtain the the beat frequency signal, it can be used to estimate the sampling locations. 

==> problem_statement.tex <==
\section{Problem Statement}
The range resolution of FMCW radar is given by - 

\begin{equation}
\Delta R = c/(2*B)
\end{equation}

where $c$ is speed of light and $B$ is the bandwidth of the signal. For mmWave FMCW radars, $B$ is generally 4 GHz and therefore the range resolution is 3.75 cm which is not sufficent to create a detailed reconstruction.

==> related_work.tex <==
\section{Related Work}



\subsection{MMwave sensing}
Millimeter-wave (mmWave) sensors, such as the Texas Instruments AWR1843BOOST, operate in the 30 GHz to 300 GHz frequency range and are capable of emitting signals that reflect off objects, capturing data on range, azimuth, elevation, intensity, and velocity. These radars are generally used for automotive applications. These are generally MIMO (Multiple-input multiple-output) radars, which means they contain multiple transmit and receive antennas.
Our system is a substantial step towards practical 3D vision using mmWave sensors.

\subsection{FMCW signals}
Frequency-Modulated Continuous-Wave (FMCW) signals are employed in radar systems to measure both the distance and velocity of targets. In FMCW radar, the transmitted signal, known as a "chirp," varies its frequency linearly over time. When this signal reflects off an object, the time delay between transmission and reception results in a frequency difference, or beat frequency, between the transmitted and received signals. This beat frequency is directly proportional to the range of the target. Additionally, any Doppler shift caused by the target's motion can be extracted to determine its velocity. FMCW radars are widely used in applications such as automotive radar systems, altimeters, and industrial sensors due to their ability to provide high-resolution measurements in a compact form factor.

\subsection{Radars}

\subsection{MIMO Radars}
Multiple-Input Multiple-Output (MIMO) radar systems employ multiple transmitting and receiving antennas to enhance detection and parameter estimation capabilities. By transmitting orthogonal waveforms from each antenna, MIMO radars can distinguish between signals reflected from various targets, enabling the construction of a virtual array with a higher number of elements than the physical array. This virtual array configuration significantly improves spatial resolution and target detection accuracy. MIMO radar systems are utilized in various applications, including automotive radar, surveillance, and remote sensing, due to their enhanced performance in complex environments.

\subsection{Neural Implicit represetation}
Neural implicit representations, also known as implicit neural representations (INRs) or neural fields, are a method of encoding continuous data, such as images, 3D shapes, or other complex signals, using neural networks. Instead of representing data through discrete structures like grids or meshes, INRs model these entities as continuous functions that map input coordinates (e.g., spatial positions) to corresponding signal values (e.g., color or density). This approach allows for the representation of intricate details and smooth variations within the data. A notable application of INRs is in 3D modeling, where techniques like Neural Radiance Fields (NeRF) utilize them for tasks such as novel view synthesis, enabling the generation of new perspectives of a scene from a limited set of images. The continuous and differentiable nature of these representations offers advantages in capturing fine details and facilitating operations like differentiation and integration over the represented space.

\subsection{Backprojection}
Classical backprojection is a foundational technique in image reconstruction, particularly in computed tomography (CT) and synthetic-aperture radar (SAR). In CT, it involves projecting collected data back into the image space along the paths of the original X-ray beams to reconstruct a visual representation of the scanned object. However, this method often results in blurred images due to the smearing effect inherent in simple backprojection. To mitigate this, filtered backprojection (FBP) is employed, which applies a filtering step to the projection data before backprojecting, thereby enhancing image clarity and resolution. Similarly, in SAR, backprojection algorithms reconstruct images by correlating received radar signals with their corresponding transmission paths, effectively focusing the data to generate high-resolution images of the target area. Despite being computationally intensive, backprojection remains a fundamental approach due to its conceptual simplicity and effectiveness in handling various imaging geometries.

